ASVspoof 2021: Towards Spoofed and Deepfake Speech Detection in the Wild

Benchmarking initiatives support the meaningful comparison of competing solutions to prominent problems in speech and language processing. Successive benchmarking evaluations typically reflect a progressive evolution from ideal lab conditions towards to those encountered in the wild. ASVspoof, the spoofing and deepfake detection initiative and challenge series, has followed the same trend. This article provides a summary of the ASVspoof 2021 challenge and the results of 54 participating teams that submitted to the evaluation phase. For the logical access (LA) task, results indicate that countermeasures are robust to newly introduced encoding and transmission effects. Results for the physical access (PA) task indicate the potential to detect replay attacks in real, as opposed to simulated physical spaces, but a lack of robustness to variations between simulated and real acoustic environments. The Deepfake (DF) task, new to the 2021 edition, targets solutions to the detection of manipulated, compressed speech data posted online. While detection solutions offer some resilience to compression effects, they lack generalization across different source datasets. In addition to a summary of the top-performing systems for each task, new analyses of influential data factors and results for hidden data subsets, the article includes a review of post-challenge results, an outline of the principal challenge limitations and a road-map for the future of ASVspoof.

==> table/DF_table.tex <==


% \begin{table}[!t]
%     \centering
%     \caption{ASVspoof 2021 progress and evaluation results for DF. Results shown in terms of pooled normalised minimum t-DCF and pooled EER [\%].}
%     \begin{tabular}{cccc}
%     \toprule
    
%           &          &    {Progress set} & {Evaluation set} \\
%       \#  & ID       &      EER          &  EER       \\ 
%     \midrule
%         1   & T23 &     0.24 &  15.64\\ 
%         2   & T20 &     1.79 &  16.05\\ 
%         3   & T08 &     2.93 &  18.30\\ 
%         4   &     &     1.65 &  18.80\\ 
%         5   & T06 &     8.29 &  19.01\\ 
%         6   & T22 &     2.17 &  19.22\\ 
%         7   & T03 &     2.32 &  19.24\\ 
%         8   & T01 &     4.72 &  19.70\\ 
%         9   & T36 &     0.78 &  20.23\\ 
%         10  & T19 &     3.00 &  20.33\\ 
%         11  & T31 &     6.88 &  20.33\\ 
%         12  &     &     2.25 &  20.63\\ 
%         13  &     &     2.00 &  20.82\\ 
%         14  & T16 &     1.98 &  20.84\\ 
%         15  &     &     4.84 &  21.61\\ 
%         16  &     &     5.06 &  21.67\\ 
%         17  &     &     2.37 &  22.03\\ 
%         18  &     &     6.10 &  22.38\\ 
%         19  & B04 &     6.10 &  22.38\\ 
%         20  & T25 &     4.18 &  22.62\\ 
%         21  & B03 &     11.61 &  23.48\\ 
%         22  &     &     0.10 &  23.57\\ 
%         23  &     &     5.36 &  23.88\\ 
%         24  & T35 &     0.42 &  24.12\\ 
%         25  &     &     11.82 &  24.89\\ 
%         26  & T30 &     4.66 &  25.21\\ 
%         27  & B02 &     21.01 &  25.25\\ 
%         28  & T26 &     16.40 &  25.41\\ 
%         29  & B01 &     17.63 &  25.56\\ 
%         30  &     &     3.40 &  26.67\\ 
%         31  & T21 &     17.20 &  28.96\\ 
%         32  &     &     9.07 &  29.25\\ 
%         33  &     &     29.63 &  29.75\\ 
%     \bottomrule
%     \end{tabular}
%     \label{tab:DF_results}
% \end{table}


==> table/DF_trial_number.tex <==
\begin{table}[!t]
    \centering
    \caption{Number of trials in each DF subset.}
    \begin{tabular}{|r|r|r|}
        \hline
        Subset & Bona fide & Spoofed \\
        \hline
        \hline
        Progress & 5,768 & 53,557  \\ 
        Evaluation & 14,869 & 5,19,059  \\ 
        \hline
    \end{tabular}
    \label{tab:DF_trial_num}
\end{table}

==> table/Hidden_trial_number.tex <==
\begin{table}[!t]
    \centering
    \caption{Number of trials in hidden subsets.}
    \begin{tabular}{|r|r|r|}
        \hline
              & Bona fide & Spoofed \\
        \hline
        \hline 
        LA  & 1,960 &  14,966   \\ 
        PA (subset 1) & 9,045 &  58,320 \\
        PA (subset 2) & 9,045 &  58,320 \\ 
        DF & 1,980 & 16,596 \\
        \hline
    \end{tabular}
    \label{tab:hidden_trial_num}
\end{table}

==> table/LA_table.tex <==

% \begin{table}[!b]
%     \centering
%     \caption{ASVspoof 2021 progress and evaluation results for LA. Results shown in terms of pooled normalised minimum t-DCF and pooled EER [\%]. \textcolor{red}{To save space, we need to consider whether remove or trim the tables. Note that progress set results are not presented anywhere else.}}
%     \begin{tabular}{cccccc}
%     \toprule
    
%           &          &    \multicolumn{2}{c}{Progress set} & \multicolumn{2}{c}{Evaluation set} \\
%     \cmidrule(lr){3-4}\cmidrule(lr){5-6}
%       \#  & ID       &     t-DCF   &  EER      & t-DCF   &  EER       \\ 
%     \midrule
%          1   &  T23 &    0.1816 &  0.89  &  0.2176 &  1.32 \\ 
%          2   &  T35 &    0.2115 &  2.61  &  0.2480 &  2.77 \\ 
%          3   &  T19 &    0.2175 &  2.69  &  0.2495 &  3.13 \\ 
%          4   &      &    0.2119 &  2.51  &  0.2500 &  2.81 \\ 
%          5   &  T36 &    0.2373 &  3.69  &  0.2531 &  3.10 \\ 
%          6   &  T20 &    0.2137 &  2.39  &  0.2608 &  3.21 \\ 
%          7   &  T08 &    0.2376 &  3.23  &  0.2672 &  3.62 \\ 
%          8   &  T16 &    0.2394 &  3.39  &  0.2689 &  3.63 \\ 
%          9   &      &    0.2436 &  3.11  &  0.2725 &  3.61 \\ 
%         10   &  T04 &    0.2372 &  4.54  &  0.2747 &  5.58 \\ 
%         11   &  T06 &    0.2476 &  5.61  &  0.2853 &  5.66 \\ 
%         12   &      &    0.2556 &  4.22  &  0.2880 &  5.01 \\ 
%         13   &  T03 &    0.2461 &  3.65  &  0.2882 &  4.66 \\ 
%         14   &      &    0.2556 &  5.90  &  0.2893 &  5.70 \\ 
%         15   &  T31 &    0.2622 &  5.00  &  0.3094 &  5.46 \\ 
%         16   &  T17 &    0.2990 &  7.10  &  0.3279 &  7.19 \\ 
%         17   &  T07 &    0.3029 &  7.88  &  0.3310 &  8.23 \\ 
%         18   &  T30 &    0.2999 &  7.58  &  0.3362 &  8.89 \\ 
%         19   &  B03 &    0.3152 &  8.90  &  0.3445 &  9.26 \\ 
%         20   &  T02 &    0.3220 &  7.71  &  0.3445 &  7.79 \\ 
%         21   &  T14 &    0.3167 &  8.82  &  0.3451 &  8.98 \\ 
%         22   &  T11 &    0.3015 &  6.80  &  0.3666 &  7.19 \\ 
%         23   &  T34 &    0.3688 &  13.25 &  0.4059 &  13.45\\ 
%         24   &  B04 &    0.4152 &  9.49  &  0.4257 &  9.50 \\ 
%         25   &  T15 &    0.2986 &  9.67  &  0.4890 &  14.68\\ 
%         26   &  B01 &    0.4948 &  15.80 &  0.4974 &  15.62\\ 
%         27   &  T25 &    0.2086 &  2.03  &  0.5148 &  13.75\\ 
%         28   &  T32 &    0.4256 &  10.93 &  0.5270 &  12.90\\ 
%         29   &      &    0.5887 &  19.04 &  0.5748 &  18.50\\ 
%         30   &  B02 &    0.5836 &  21.13 &  0.5758 &  19.30\\ 
%         31   &      &    0.2528 &  5.26  &  0.5775 &  14.28\\ 
%         32   &  T01 &    0.2773 &  6.32  &  0.6204 &  15.95\\ 
%         33   &      &    0.2792 &  7.87  &  0.6288 &  15.87\\ 
%         34   &  T24 &    0.3108 &  10.85 &  0.6320 &  15.98\\ 
%         35   &      &    0.3233 &  9.72  &  0.6370 &  16.27\\ 
%         36   &  T29 &    0.3316 &  11.87 &  0.6741 &  17.41\\ 
%         37   &      &    0.3679 &  12.54 &  0.6812 &  17.66\\ 
%         38   &  T12 &    0.6900 &  26.26 &  0.7227 &  26.41\\ 
%         39   &      &    0.4382 &  13.77 &  0.7233 &  19.19\\ 
%         40   &      &    0.6123 &  23.16 &  0.8521 &  26.14\\ 
%         41   &      &    0.9988 &  53.16 &  1.0000 &  53.81\\  
%     \bottomrule
%     \end{tabular}
%     \label{tab:LA_results}
% \end{table}


==> table/LA_trial_number.tex <==
\begin{table}[!t]
    \centering
    \caption{Number of trials in each LA subset.}
    \begin{tabular}{|r|r|r|}
        \hline
        Subset & Bona fide & Spoofed \\
        \hline
        \hline
        Progress & 1,676 & 14,788  \\ 
        Evaluation & 14,816 & 133,360  \\ 
        %Hidden track & 1,960 &  14,966 \\
        \hline
    \end{tabular}
    \label{tab:LA_trial_num}
\end{table}

==> table/PA_condition_per_ASVroom.tex <==
\begin{table}[t]
    \centering
    \caption{Summary of PA data conditions. }
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|c|c|}
    R1 & r1m1d4s2 r1m2d2s2 r1m3d3s2 r2m1d2s2 r2m2d3s2 r2m3d4s2 r3m1d3s2 r3m2d4s2 r3m3d2s2  \\
R2 & r1m1d4s3 r1m2d2s3 r1m3d3s3 r2m1d2s3 r2m2d3s3 r2m3d4s3 r3m1d3s3 r3m2d4s3 r3m3d2s3   \\
R3 & r1m1d4s4 r1m2d2s4 r1m3d3s4 r2m1d2s4 r2m2d3s4 r2m3d4s4 r3m1d3s4 r3m2d4s4 r3m3d2s4   \\
R4 & r4m1d4s2 r4m2d2s2 r4m3d3s2 r5m1d2s2 r5m2d3s2 r5m3d4s2 r6m1d3s2 r6m2d4s2 r6m3d4s2   \\
R5 & r4m1d4s3 r4m2d2s3 r4m3d3s3 r5m1d2s3 r5m2d3s3 r5m3d4s3 r6m1d3s3 r6m2d4s3 r6m3d2s3   \\
R6 & r4m1d4s4 r4m2d2s4 r4m3d3s4 r5m1d2s4 r5m2d3s4 r5m3d4s4 r6m1d3s4 r6m2d4s4 r6m3d2s4   \\
R7 & r7m1d4s3 r7m2d2s3 r7m3d3s3 r8m1d2s3 r8m2d3s3 r8m3d4s3 r9m1d3s3 r9m2d4s3 r9m3d2s3   \\
R8 & r7m1d4s2 r7m2d2s2 r7m3d3s2 r8m1d2s2 r8m2d3s2 r8m3d4s2 r9m1d3s2 r9m2d4s2 r9m3d2s2   \\
R9 & r7m1d4s4 r7m2d2s4 r7m3d3s4 r8m1d2s4 r8m2d3s4 r8m3d4s4 r9m1d3s4 r9m2d4s4 r9m3d2s4
    \end{tabular}
    }
    \end{table}

==> table/PA_condition_table1.tex <==

\begin{table}[t]
    \centering
    \caption{Summary of PA evaluation conditions. }
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|c|c|c| c |c|c|c|}
        \cline{1-3}
         & \multirow{2}{*}{Cond.}   & Room size & \multicolumn{4}{c}{} \\ 
        \cline{5-7}
         &  & $w\times d \times h (m)$ &  & & Cond. & Angle, Dis.(m)  \\ 
        \cline{1-3}\cline{5-7}
        \multirow{9}{1.2cm}{$S_{\text{asv}}$ / $S_{\text{a}}$} & R1 / r1 & $8.0\times8.0\times2.4$ &  & \multirow{6}{1.cm}{$D_{s}$, $D_{s}'$}    & D1 & $15^{\circ}$,  2.0  \\ 
                                                             & R2 / r2 & $6.0\times5.0\times2.3$ &  &                                           & D2 & $45^{\circ}$,  1.5  \\ 
                                                             & R3 / r3 & $6.6\times5.0\times2.4$ &  &                                           & D3 & $75^{\circ}$,  1.0  \\
                                                             & R4 / r4 & $7.5\times7.7\times2.6$ &  &                                           & D4 & $90^{\circ}$,  0.5  \\
                                                             & R5 / r5 & $7.2\times4.0\times2.3$ &  &                                           & D5 & $120^{\circ}$, 1.25 \\
                                                             & R6 / r6 & $4.5\times6.5\times2.5$ &  &                                           & D6 & $150^{\circ}$, 1.75 \\
        \cline{5-7}
                                                             & R7 / r7 & $4.5\times2.4\times2.4$ &  & \multirow{3}{*}{$D_{a}$}   & d2 & $45^{\circ}$,  1.5  \\ %$45^{\circ}$,  1.5
                                                             & R8 / r8 & $7.1\times4.8\times2.5$ &  &                            & d3 & $75^{\circ}$,  1.0  \\ %$75^{\circ}$,  1.0
                                                             & R9 / r9 & $5.9\times4.0\times2.8$ &  &                            & d4 & $90^{\circ}$,  0.5  \\ %$90^{\circ}$,  0.5
        \cline{1-3} \cline{5-7}
        \multicolumn{7}{c}{} \\ 
        \cline{1-3} \cline{5-7}
        &  Cond. &  Mic. type &  & & Cond. & Device type \\ 
        \cline{1-3} \cline{5-7}
        \multirow{3}{1.2cm}{$Q_{\text{asv,m}}$ / $Q_{\text{a,m}}$} & M1/m1 & MPM-1000 (condenser)  & & \multirow{3}{*}{$Q_{a, s}$}  & s2 & SONY \\
                                                                    & M2/m2 & Uber Mic (condenser) & &  & s3 & NEUMANN \\
                                                                    & M3/m3  & iPad Air (MEMS)  & &  & s4 & GENELEC \\
        \cline{1-3}\cline{5-7}
    \end{tabular}
    }
    \label{tab:PA_conditions}
\end{table}

==> table/PA_device.tex <==
% \begin{table}[!t]
%     \centering
%     \caption{Details on microphone and replay devices used in PA data recording. Numbers are from official specifications. }
%     \begin{tabular}{lccc}
%     \toprule
%     Replay device       & s2 & s3 & s4 \\
%     \midrule
%     \multirow{2}{*}{Brand} & SONY & NEUMANN & GENELC \\
%           & SRS-XB43 & KH 80 DSP & 8030 CP \\
%     \shortstack[l]{Lower cut-off \\ freq. (–6 dB) in Hz} & 20 & 53 & 47 \\
%     \shortstack[l]{Upper cut-off \\ freq. (–6 dB) in Hz} & 20k & 22k & 25k \\
%     \shortstack[l]{Passband free-field \\ FR ($\pm$ 2dB) in Hz} & UNAVAL. & 59 - 20k & 54 - 20k \\
%     \bottomrule
%     & \\
%     \toprule
%     Microphone       & M1/m1 & M2/m2 & M3/m3 \\
%     \midrule
%     \multirow{2}{*}{Brand}  & Marantz & M-Audio &  iPad Air\\
%                             & MPM-1000 & Uber-mic & MEMS mic. \\
%     FR in Hz &  20 - 20k & 30 - 20k & UNAVAIL. \\
%     SNR  in dB & 77 & 110 & UNAVAIL. \\
%     Sensitivity in dB & 45 & 38 ($\pm$ 2)& UNAVAIL.\\
%     \bottomrule
%     \end{tabular}
%     \label{tab:PA_device}
% \end{table}

% \begin{comment}
% GENELEC: https://www.genelec.jp/studio-monitors/classic-studio-monitors-subwoofers/8030-studio-monitor/
% https://assets.ctfassets.net/4zjnzn055a4v/1my4dzvqUoe4oKYwS6KsUu/a8f964c3ce07eb802b88b8d861799a07/8030c_opman_gb_fi.pdf
% NEUMMAN: https://www.neumann.com/homestudio/en/kh-80
% SONY: https://www.sony.jp/active-speaker/products/SRS-XB43/
% Marantz: MPM-1000 http://marantzpro.jp/mpm-1000/
% http://www.marantzpro.jp/mpm-1000/data/mpm-1000_userguide_v1.0-jp.pdf
% M-audio: https://www.m-audio.com/ubermic
% \end{comment}

==> table/PA_table.tex <==

% \begin{table}[!t]
%     \centering
%     \caption{ASVspoof 2021 progress and evaluation results for PA. Results shown in terms of pooled normalised minimum t-DCF and pooled EER [\%].}
%     \begin{tabular}{cccccc}
%     \toprule
    
%           &          &    \multicolumn{2}{c}{Progress set} & \multicolumn{2}{c}{Evaluation set} \\
%     \cmidrule(lr){3-4}\cmidrule(lr){5-6}
%       \#  & ID       &     t-DCF   &  EER      & t-DCF   &  EER       \\ 
%     \midrule
%     1   & T07 &     0.6736 &  23.60 &  0.6824 &  24.25\\ 
%     2   & T16 &     0.6790 &  25.37 &  0.7122 &  27.59\\ 
%     3   & T23 &     0.7019 &  24.22 &  0.7296 &  26.42\\ 
%     4   & T01 &     0.6925 &  25.73 &  0.7446 &  28.36\\ 
%     5   & T04 &     0.6676 &  24.80 &  0.7462 &  29.00\\ 
%     6   &     &     0.7207 &  27.23 &  0.7469 &  29.22\\ 
%     7   & T33 &     0.7263 &  27.00 &  0.7648 &  29.55\\ 
%     8   & T08 &     0.7177 &  25.95 &  0.7670 &  29.02\\ 
%     9   & T37 &     0.7912 &  32.39 &  0.8216 &  35.07\\ 
%     10   & T27 &     0.8102 &  31.62 &  0.8307 &  32.00\\ 
%     11   & T26 &     0.7837 &  26.91 &  0.8362 &  29.61\\ 
%     12   & T28 &     0.8498 &  30.94 &  0.8879 &  32.96\\ 
%     13   &     &     0.8934 &  35.16 &  0.9265 &  37.10\\ 
%     14   & B01 &     0.9062 &  36.33 &  0.9434 &  38.07\\ 
%     15   & T03 &     0.9084 &  36.37 &  0.9444 &  38.07\\ 
%     16   &     &     0.9193 &  35.78 &  0.9530 &  38.50\\ 
%     17   & T09 &     0.9531 &  34.39 &  0.9666 &  34.77\\ 
%     18   & B02 &     0.9747 &  39.79 &  0.9724 &  39.54\\ 
%     19   & T11 &     0.9836 &  40.91 &  0.9939 &  42.55\\ 
%     20   &     &     0.9855 &  40.38 &  0.9945 &  42.98\\ 
%     21   & B03 &     0.9827 &  42.16 &  0.9958 &  44.77\\ 
%     22   & B04 &     0.9993 &  46.03 &  0.9997 &  48.60\\ 
%     23   & T10 &     0.9996 &  45.10 &  1.0000 &  45.50\\ 
%     \bottomrule
%     \end{tabular}
%     \label{tab:PA_results}
% \end{table}

==> table/PA_trial_number.tex <==
\begin{table}[!t]
    \centering
    \caption{Number of trials in each PA subset.}
    \begin{tabular}{|r|r|r|}
        \hline
        Subset & Bona fide & Spoofed \\
        \hline
        \hline
        Progress & 14,472 & 72,576  \\ 
        Evaluation & 94,068 & 627,264  \\ 
        %Hidden track 1 & 9,045 &  58,320 \\
        %Hidden track 2 & 9,045 &  58,320 \\ 
        \hline
    \end{tabular}
    \label{tab:PA_trial_num}
\end{table}
